P6: A Declarative Language for Integrating Machine Learning in Visual Analytics

We present P6, a declarative language for building high performance visual analytics systems through its support for specifying and integrating machine learning and interactive visualization methods. As data analysis methods based on machine learning and artificial intelligence continue to advance, a visual analytics solution can leverage these methods for better exploiting large and complex data. However, integrating machine learning methods with interactive visual analysis is challenging. Existing declarative programming libraries and toolkits for visualization lack support for coupling machine learning methods. By providing a declarative language for visual analytics, P6 can empower more developers to create visual analytics applications that combine machine learning and visualization methods for data analysis and problem solving. Through a variety of example applications, we demonstrate P6's capabilities and show the benefits of using declarative specifications to build visual analytics systems. We also identify and discuss the research opportunities and challenges for declarative visual analytics.

==> Sections/6Opportunities.tex <==
\section{Opportunities and Challenges}
Our work is only an initial step toward declarative visual analytics.
We have identified opportunities and challenges for further research.

\subsection{Progressive Visual Analytics}
Progressive visual analytics provides an effective way for interactive analysis of big data.
By delivering incremental results to maintain an acceptable level of responsiveness, progressive visual analytics systems allow users to interact with the intermediate results and steer the analysis process.
Several systems~\cite{stolper2014progressive,badam2017steering,pezzotti2018deepeyes} have been developed by researchers to prove the usefulness of progressive visual analytics.
In addition, researchers have developed several frameworks~\cite{muhlbacher2014opening,schulz2016enhanced,turkay2017designing} to provide progressive visual analytics system design guideline, and conducted user studies~\cite{Fisher2012,zgraggen2017progressive} to show that progressive visual analytics can lead to more insights and better experience for interactive visual analysis.

Many machine learning algorithms have high computational complexity, which become slow when executing on large datasets.
Therefore, integrating machine learning with progressive visual analytics can better facilitate interactive analysis of big data.
While not all machine learning methods can generate meaningful incremental or partial results, researchers in visual analytics and machine learning should collaborate to adapt more methods to support progressive data analysis.
For machine learning methods that can produce meaningful incremental results, declarative grammars can be designed for specifying how to use these methods for progressive and interactive visual analysis.

In P5~\cite{li2019p5}, we have developed a declarative language for progressive visualization, but it lacks support for using machine learning methods for advanced data analysis.
A declarative language for integrating incremental machine learning methods with progressive visual analytics can provide great value to researchers and developers.
System development can be benefited by providing rapid specifications for how to execute machine learning methods progressively, visualize the incremental results, adjust parameters in both the machine learning methods, and steer the visual analysis process.

\subsection{Collaborative Visual Analytics}
Enabling collaboration was identified as a major challenge for the field of visual analytics~\cite{cook2005illuminating,isenberg2011collaborative}.
A large amount of work provided system design guidelines~\cite{wattenberg2006designing,heer2007voyagers,viegas2007manyeyes,heer2008design,mahyar2014supporting}, software infrastructure~\cite{badam2014polychrome,mcgrath2012branch,li2015high}, and user behavior studies~\cite{isenberg2008exploratory,robinson2008collaborative,isenberg2010exploratory} for collaborative visual analysis.

Recent work~\cite{li2020resolving} has shown that using a declarative visualization language for collaborative data analysis allows better understanding of the shared visualizations among a team of analysts and encourages analysts to build on each other's findings.
Therefore, we expect that adopting a declarative visual analytics language in collaborative data analysis to be beneficial too. 
Adopting declarative languages in such a context opens several research opportunities.
First, we need to develop methods to effectively generate annotations on the visualizations of analysis results based on machine learning methods.
This allows better externalization of insights from visualization and sharing for collaborative data analysis.
Second, it is possible to develop mechanisms for automatically combining analysis results in declarative specifications from multiple analysts.
The combined results can be visualized to examine all the findings and analyze the coverage of exploration~\cite{xu2018chart}.
From the combined results, we can identify and indicate common findings among multiple analysts, because these overlapping findings usually are important insights~\cite{Chung2010-xd,mahyar2014supporting}.
In addition, we can employ existing revision control systems (e.g., Git) for tracking the changes in declarative specifications as well as detecting conflicts in the findings from different analysts.
Identifying conflicting insights in collaborative sensemaking can  often lead to better analysis results~\cite{li2020resolving}.
We believe that developing and incorporating these methods in declarative languages can better facilitate collaborative data analysis and sense making.

% \subsection{Design Models}
% Revisit interaction taxonomies, models, and frameworks.
% Add a level or categories for interactive machine learning and human-machine collaboration. 
% Decide what tasks should be human assisting machines, and what tasks should be AI assisting human.

\subsection{Debugging and Deployment}
A well-known drawback of declarative languages is that debugging is difficult as internal structures and executions are not exposed to programmers~\cite{bostock2011d3, satyanarayan2016reactive}.
While the benefits of declarative languages outweight this difficulty, developing effective tools to support debugging declarative specifications of visual analytics applications can remove this disadvantage entirely.
For example, Hoffswell et al.~\cite{hoffswell2016visual} have developed a visual debugging tool for declarative data visualization.
Their approach can be adopted and extended for debugging visual analytics applications that are developing with declarative specifications.

In addition to debugging, support for deploying a visual analytics application on different platforms and clouding computing services can be added in declarative languages.
Before transiting to production, the development can use a local computing environment that is easier for debugging.
When the system is ready to deploy for experimental or production use, the declarative specification for deployment can be used to automatically build and upload the application to the targeted platform.

\subsection{Toward Visual Analytics as Services}
When using the P6 declarative language for building a visual analytics system, 
programmers do not need to deal with the complexity of setting up the backend server or remote computing services.
This approach can be extended to support visual analytics as services that leverage cloud computing for performing data processing and machine learning computations.  
The operations in the declarative specifications are executed at runtime using cloud computing services.
Cloud computing can dynamically allocate computing instances based on the declarative specifications, providing  better scalability and availability for hosting visual analytics applications. 
We can extend the declarative language for requesting cloud computing resources based on the data size and computational complexity.
The request can be specified using the response time requirements for visual analysis tasks based on appropriate human computer interaction models~\cite{card1983psychology,card1999readings} and recent user study~\cite{liu2014effects}.
Providing visual analytics as services can make building scalable systems easier and allow better utilization of computing resources.

==> VGTC/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> VGTC/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

